Adaptive Correspondence Scoring for Unsupervised Medical Image Registration

We propose an adaptive training scheme for unsupervised medical image registration. Existing methods rely on image reconstruction as the primary supervision signal. However, nuisance variables (e.g. noise and covisibility), violation of the Lambertian assumption in physical waves (e.g. ultrasound), and inconsistent image acquisition can all cause a loss of correspondence between medical images. As the unsupervised learning scheme relies on intensity constancy between images to establish correspondence for reconstruction, this introduces spurious error residuals that are not modeled by the typical training objective. To mitigate this, we propose an adaptive framework that re-weights the error residuals with a correspondence scoring map during training, preventing the parametric displacement estimator from drifting away due to noisy gradients, which leads to performance degradation. To illustrate the versatility and effectiveness of our method, we tested our framework on three representative registration architectures across three medical image datasets along with other baselines. Our adaptive framework consistently outperforms other methods both quantitatively and qualitatively. Paired t-tests show that our improvements are statistically significant. Code available at: \url{https://voldemort108x.github.io/AdaCS/}.

==> tables/ablation_table.tex <==
\begin{table}[tb]
    \caption{Ablation study on loss terms. Note: Removing $\mathcal{L}_{\text{reg}}$ leads to a degenerate solution of all-zeros for the scoring estimator $g_\phi(\cdot)$.}
    \centering
    \begin{adjustbox}{scale=0.6}
    % \begin{subtable}{0.4\linewidth}
    % \centering
        \begin{tabular}{lccccccccc}
            \toprule 
            & \multicolumn{2}{c}{Loss} & \multicolumn{3}{c}{ACDC \cite{bernard_deep_2018}} & \multicolumn{3}{c}{CAMUS \cite{leclerc_deep_2019}}  \\
            
            \cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-9} 
            
            & $\mathcal{L}_{\text{reg}}$ & $\revise{\mathcal{L}_{\text{smooth}}}$  & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$  \\\midrule
            \midrule
            
            \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{vxm}}} & \cmark & \xmark
              & 80.24 & \textbf{4.64} & 1.23 & 81.58 & 8.89 & 1.74  \\
            & \cmark & \cmark & \textbf{80.50} & 4.69 & \textbf{1.23} & \textbf{81.74} & \textbf{8.55} & \textbf{1.72}  \\
            \midrule 
        
            \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\small tsm}}}
            & \cmark & \xmark & 77.84 & 5.41 & 1.33 & 79.58 & 10.17 & 1.81  \\
            & \cmark & \cmark & \textbf{78.39} & \textbf{5.40} & \textbf{1.32} & \textbf{79.64} & \textbf{9.85} & \textbf{1.79}  \\
            \midrule 
            
            \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\small dfm}}}
            & \cmark & \xmark & 71.62 & 5.56 & 1.58 & 77.32 & 9.71 & 2.00  \\
            & \cmark & \cmark & \textbf{72.09} & \textbf{5.35} & \textbf{1.53} & \textbf{77.65} & \textbf{9.82} & \textbf{1.99}  \\
            \bottomrule 
        \end{tabular}
    % \end{subtable}
    \end{adjustbox}%
    \label{tab:ablation_table}
\end{table}

% \begin{table}[htbp]
%     \vspace{-1mm}
%     \centering
%     \begin{adjustbox}{scale=0.5}
%     \begin{tabular}{llccccccc}
%     \toprule 
%     & & \multicolumn{3}{c}{ACDC} & \multicolumn{3}{c}{CAMUS} \\
    
%     \cmidrule(lr){3-5} \cmidrule(lr){6-8}
    
%     & & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$  \\\midrule
%     \midrule
    
%     \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\small vxm}}}
%     & w/o $m_T$   & 80.00 & 4.71 & 1.24 & 81.27 & 8.86 & 1.76  \\
%     & w. $m_T$  & \textbf{80.50} & \textbf{4.69} & \textbf{1.23} & \textbf{81.74} & \textbf{8.55} & \textbf{1.72} \\\midrule
    
%     \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\small tsm}}}
%     & w/o $m_T$   & 77.12 & 5.65 & \textbf{1.32} & 79.43 & \textbf{9.85} & \textbf{1.79}  \\
%     & w. $m_T$  & \textbf{78.39} & \textbf{5.40} & \textbf{1.32} & \textbf{79.64} & \textbf{9.85} & \textbf{1.79} \\\midrule
    
%     \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\small dfm}}}
%     & w/o $m_T$   & 71.62 & 5.56 & 1.58 & 77.28 & \textbf{9.61} & 2.00  \\
%     & w. $m_T$  & \textbf{72.09} & \textbf{5.35} & \textbf{1.53} & \textbf{77.65} & 9.82 & \textbf{1.99} \\
%     \bottomrule 
    
%     \end{tabular}
%     \end{adjustbox}
%     % \caption{Ablation on momentum-guided weighting $m_T$.}
%     \label{tab:rebuttal_ablation}
%     \vspace{-2mm}
% \end{table}

==> tables/contour_table.tex <==
\begin{table}[tb]
    \caption{\revise{Contour-based metrics compared against baselines. Units: DSC (\%) HD (vx) ASD (vx). Our method consistently improves on registration accuracy across different architectures and datasets.}}
    \centering
    \begin{adjustbox}{scale=0.9}
    \begin{tabular}{llccccccc}
    \toprule 
    & & \multicolumn{3}{c}{ACDC \cite{bernard_deep_2018}} & \multicolumn{3}{c}{CAMUS \cite{leclerc_deep_2019}} \\
    
    \cmidrule(lr){3-5} \cmidrule(lr){6-8}
    
    & & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$  \\\midrule
    \midrule
    % & Undeformed & 47.98 & 7.91 & 2.32 & 66.77 & 10.87 & 2.61 \\ \midrule
    % & Elastix & 77.26 & 4.95 & 1.28 & 80.18 & 10.02 & 1.81 \\\midrule
    
    \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\small CNN}}}
    & Voxelmorph \cite{balakrishnan_voxelmorph_2019} & 79.48 & 4.79 & 1.27 & 81.50 & 8.72 & 1.74  \\
    & NLL \cite{kendall_what_2017}                      & 76.49 & 5.46 & 1.45 & 75.24 & 11.05 & 2.20  \\
    & $\beta$-NLL \cite{seitzer_pitfalls_2022}          & 78.74 & 5.07 & 1.33 & 79.75 &  9.39 & 1.93  \\
    & AdaFrame \cite{wong_adaptive_2021} & 66.38 & 5.80 & 1.67 & 77.88 & 10.54 & 1.93  \\
    & AdaReg \cite{wong_bilateral_2019} & 78.75 & 5.13 & 1.33 & 79.31 & 9.78 & 1.88  \\
    & AdaCS (Ours) & \textbf{80.50} & \textbf{4.69} & \textbf{1.23} & \textbf{81.74} & \textbf{8.55} & \textbf{1.72} \\
    \midrule 

    \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\small Transformer}}}
    & Transmorph \cite{chen_transmorph_2022} & 76.94 & 5.51 & 1.30 & 79.24 & 10.30 & \textbf{1.79}  \\
    & NLL \cite{kendall_what_2017}                      & 73.12 & 7.22 & \textbf{1.27} & 75.08 & 11.60 & \textbf{1.79}  \\
    & $\beta$-NLL \cite{seitzer_pitfalls_2022}          & 75.74 & 6.12 & 1.29 & 77.39 & 10.99 & 1.86  \\
    & AdaFrame \cite{wong_adaptive_2021} & 67.95 & 5.72 & 1.59 & 78.06 & 9.86 & 1.91  \\
    & AdaReg \cite{wong_bilateral_2019} & 76.22 & 5.68 & 1.29 & 78.12 & 10.62 & 1.84  \\
    & AdaCS (Ours) & \textbf{78.39} & \textbf{5.40} & 1.32 & \textbf{79.64} & \textbf{9.85} & \textbf{1.79}  \\
    \midrule 
    
    \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\small Diffusion}}}
    & Diffusemorph \cite{kim_diffusemorph_2022} & 67.38 & 5.80 & 1.67 & 75.23 & \textbf{9.80} & 2.07  \\
    & NLL \cite{kendall_what_2017}                      & 66.24 & 5.84 & 1.73 & 74.78 & 10.62 & 2.15  \\
    & $\beta$-NLL \cite{seitzer_pitfalls_2022}          & 66.31 & 5.93 & 1.74 & 73.27 & 9.85 & 2.25  \\
    & AdaFrame \cite{wong_adaptive_2021} & 59.78 & 6.46 & 1.93 & 75.04 & 10.41 & 2.10  \\
    & AdaReg \cite{wong_bilateral_2019} & 69.41 & 6.25 & 1.78 & 74.36 & 10.66 & 2.21  \\
    & AdaCS (Ours) & \textbf{72.09} & \textbf{5.35} & \textbf{1.53} & \textbf{77.65} & 9.82 & \textbf{1.99} \\
    \bottomrule 
    \end{tabular}
    \end{adjustbox}
    \label{tab:contour_table}
\end{table}
% \begin{table}[tb]
%     \caption{Contour-based metrics compared against baselines. Units: DSC (\%) HD (vx) ASD (vx). Our method consistently improves on registration accuracy across different architectures and datasets.}
%     \centering
%     \begin{adjustbox}{scale=0.6}
%     \revise{
%     \begin{tabular}{lcccccc|cccccc|cccccc}
%     \toprule 
%     % & \multicolumn{6}{c}{Voxelmorph-based \cite{balakrishnan_voxelmorph_2019}} \\
%     % \cmidrule(lr){2-7}
    
%     & \multicolumn{3}{c}{ACDC} & \multicolumn{3}{c}{CAMUS } & \multicolumn{3}{c}{ACDC} & \multicolumn{3}{c}{CAMUS} & \multicolumn{3}{c}{ACDC} & \multicolumn{3}{c}{CAMUS} \\
    
%     \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
    
%     & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$  \\\midrule
%     \midrule
%     % & Undeformed & 47.98 & 7.91 & 2.32 & 66.77 & 10.87 & 2.61 \\ \midrule
%     % & Elastix & 77.26 & 4.95 & 1.28 & 80.18 & 10.02 & 1.81 \\\midrule
%     & \multicolumn{6}{c}{Voxelmorph-based \cite{balakrishnan_voxelmorph_2019}} & \multicolumn{6}{c}{Transmorph-based \cite{chen_transmorph_2022}} & \multicolumn{6}{c}{Diffusemorph-based \cite{kim_diffusemorph_2022}}\\
%     \cmidrule(lr){2-7}
%     MSE \cite{balakrishnan_voxelmorph_2019}     & 79.48 & 4.79 & 1.27 & 81.50 & 8.72 & 1.74 & 76.94 & 5.51 & 1.30 & 79.24 & 10.30 & \textbf{1.79} &   67.38 & 5.80 & 1.67 & 75.23 & \textbf{9.80} & 2.07\\
%     NLL \cite{kendall_what_2017}                      & 76.49 & 5.46 & 1.45 & 75.24 & 11.05 & 2.20  \\
%     $\beta$-NLL \cite{seitzer_pitfalls_2022}          & 78.74 & 5.07 & 1.33 & 79.75 &  9.39 & 1.93  \\
%     AdaFrame \cite{wong_adaptive_2021} & 66.38 & 5.80 & 1.67 & 77.88 & 10.54 & 1.93  \\
%     AdaReg \cite{wong_bilateral_2019} & 78.75 & 5.13 & 1.33 & 79.31 & 9.78 & 1.88  \\
%     AdaCS (Ours) & \textbf{80.50} & \textbf{4.69} & \textbf{1.23} & \textbf{81.74} & \textbf{8.55} & \textbf{1.72} \\
%     \midrule 

%     Transmorph \cite{chen_transmorph_2022} & 76.94 & 5.51 & 1.30 & 79.24 & 10.30 & \textbf{1.79}  \\
%     NLL \cite{kendall_what_2017}                      & 73.12 & 7.22 & \textbf{1.27} & 75.08 & 11.60 & \textbf{1.79}  \\
%     $\beta$-NLL \cite{seitzer_pitfalls_2022}          & 75.74 & 6.12 & 1.29 & 77.39 & 10.99 & 1.86  \\
%     AdaFrame \cite{wong_adaptive_2021} & 67.95 & 5.72 & 1.59 & 78.06 & 9.86 & 1.91  \\
%     AdaReg \cite{wong_bilateral_2019} & 76.22 & 5.68 & 1.29 & 78.12 & 10.62 & 1.84  \\
%     AdaCS (Ours) & \textbf{78.39} & \textbf{5.40} & 1.32 & \textbf{79.64} & \textbf{9.85} & \textbf{1.79}  \\
%     \midrule 
    
%     Diffusemorph \cite{kim_diffusemorph_2022} & 67.38 & 5.80 & 1.67 & 75.23 & \textbf{9.80} & 2.07  \\
%     NLL \cite{kendall_what_2017}                      & 66.24 & 5.84 & 1.73 & 74.78 & 10.62 & 2.15  \\
%     $\beta$-NLL \cite{seitzer_pitfalls_2022}          & 66.31 & 5.93 & 1.74 & 73.27 & 9.85 & 2.25  \\
%     AdaFrame \cite{wong_adaptive_2021} & 59.78 & 6.46 & 1.93 & 75.04 & 10.41 & 2.10  \\
%     AdaReg \cite{wong_bilateral_2019} & 69.41 & 6.25 & 1.78 & 74.36 & 10.66 & 2.21  \\
%     AdaCS (Ours) & \textbf{72.09} & \textbf{5.35} & \textbf{1.53} & \textbf{77.65} & 9.82 & \textbf{1.99} \\
%     \bottomrule 
%     \end{tabular}
%     }
%     \end{adjustbox}
%     \label{tab:contour_table}
% \end{table}

==> tables/loss_ablation.tex <==
\begin{table}[tb]
    \caption{Comparison with other robust loss functions (NCC, MI).}
    \centering
    \begin{adjustbox}{scale=1}
                \begin{tabular}{llccccccc}
                    \toprule 
                    & & \multicolumn{3}{c}{ACDC \cite{bernard_deep_2018}} & \multicolumn{3}{c}{CAMUS \cite{leclerc_deep_2019}} \\
                    \cmidrule(lr){3-5} \cmidrule(lr){6-8}
                    
                    & & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$  \\\midrule
                    \midrule
                    
                    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\small vxm}}}
                    & NCC  & 78.55 & 4.94 & 1.29 & 77.01 & 10.23 & 1.89  \\
                    & MI   & 78.04 & 5.25 & 1.35 & 78.18 & 9.83 & 1.99  \\
                    & MSE  & 79.48 & 4.79 & 1.27 & 81.50 & 8.72 & 1.74 \\
                    & AdaCS & \textbf{80.50} & \textbf{4.69} & \textbf{1.23} & \textbf{81.74} & \textbf{8.55} & \textbf{1.72} \\\midrule
                    
                    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\small tsm}}}
                    & NCC  & 73.77 & 6.64 & 1.12 & 73.03 & 11.87 & \textbf{1.70}  \\
                    & MI   & 73.57 & 6.57 & \textbf{1.11} & 74.83 & 11.94 & 1.83  \\
                    & MSE  & 76.94 & 5.51 & 1.30 & 79.24 & 10.30 & 1.79  \\
                    & AdaCS & \textbf{78.39} & \textbf{5.40} & 1.32 & \textbf{79.64} & \textbf{9.85} & 1.79  \\\midrule
                    
                    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\small dfm}}}
                    & NCC  & 70.25 & \textbf{5.29} & 1.58 & 75.67 & 10.75 & 2.06  \\
                    & MI   & 71.16 & 5.40 & 1.56 & 76.19 & 10.09 & 2.16  \\
                    & MSE  & 67.38 & 5.80 & 1.67 & 75.23 & \textbf{9.80} & 2.07  \\
                    & AdaCS & \textbf{72.09} & 5.35 & \textbf{1.53} & \textbf{77.65} & 9.82 & \textbf{1.99}   \\
                    \bottomrule 
                    \end{tabular}
    \end{adjustbox}
    \label{tab:loss_ablation}
\end{table}

==> tables/p_values_table.tex <==
\begin{table}[tb]
    \caption{\revise{Paired t-test of our proposed method v.s. second-best method in \cref{tab:contour_table} for each dataset in terms of DSC. The p-values suggested that our improvement is statistically significant.}}
    \centering
    \begin{adjustbox}{scale=0.8}
    \begin{tabular}{lccc}
    \toprule 
    & Voxelmorph \cite{balakrishnan_voxelmorph_2019} & Transmorph \cite{chen_transmorph_2022} & Diffusemorph \cite{kim_diffusemorph_2022} \\\midrule\midrule
    ACDC \cite{bernard_deep_2018} & $p=5.85\times 10^{-16}$ & $p=0.046$ & $p=1.01\times 10^{-41}$\\
    CAMUS \cite{leclerc_deep_2019} & $p=0.01$ & $p=0.01$ & $p=4.56\times 10^{-41}$\\
    \bottomrule
    
    \end{tabular}
    \end{adjustbox}
    \label{tab:p_values}
\end{table}
